Centre vortex structure in the presence of dynamical fermions

An analysis of the geometry and structure of centre vortices in the presence of dynamical fermions is performed. A variety of metrics are used to measure the matrix structure of the vortex-modified gauge fields. Visualisations of centre vortices are presented and percolating clusters are identified. The size of secondary vortex clusters is analysed, with substantial differences observed between the pure Yang-Mills and dynamical fermion case. Vortex fields are represented as directed graphs, with branching points acting as the vertices. This representation leads to a novel picture of vortex branching as a binomial process. These results elucidate the change in the centre vortex vacuum induced by the introduction of dynamical fermions.

==> include/PG_loop_table.tex <==
 & $\hat{x}$ & $\hat{y}$ & $\hat{z}$ & $\hat{t}$ \\ 
 \hline\\
$N_{\rm total}$ & 3285(6) & 3281(6) & 3286(6) & 1645(3) \\
$N_{\rm primary}$ & 3278(6) & 3273(6) & 3279(6) & 1638(3) \\
$N_{\rm secondary}$ & 7.34(5) & 7.48(5) & 7.40(5) & 7.32(5) \\


==> include/heavy_loop_table.tex <==
 & $\hat{x}$ & $\hat{y}$ & $\hat{z}$ & $\hat{t}$ \\ 
 \hline\\
$N_{\rm total}$ & 6.51e+03(7) & 6.54e+03(6) & 6.49e+03(7) & 3.27e+03(4) \\
$N_{\rm primary}$ & 6.50e+03(7) & 6.53e+03(6) & 6.48e+03(7) & 3.27e+03(4) \\
$N_{\rm secondary}$ & 5.132(9) & 5.09(4) & 5.08(1) & 4.968(7) \\


==> include/light_loop_table.tex <==
 & $\hat{x}$ & $\hat{y}$ & $\hat{z}$ & $\hat{t}$ \\ 
 \hline\\
$N_{\rm total}$ & 5929(9) & 5930(9) & 5933(9) & 2969(4) \\
$N_{\rm primary}$ & 5924(9) & 5925(9) & 5928(9) & 2964(4) \\
$N_{\rm secondary}$ & 5.014(5) & 5.020(5) & 5.020(5) & 5.011(5) \\


==> include/rate_fit_table.tex <==
Ensemble & \mc{$q_{\rm fit}$} & \mc{$\lambda_{\rm fit}~(\si{fm^{-1}})$} & \mc{$\alpha$} & \mc{$\beta$} \\
\midrule
Pure gauge & 0.067(1) & 0.67(1) & 0.0805(1) & 0.0774(1) \\
\mc{$701~\si{MeV}$} & 0.100(1) & 0.98(1) & 0.1499(1) & 0.13971(1) \\
\mc{$156~\si{MeV}$} & 0.092(2) & 0.99(2) & 0.1417(1) & 0.1326(1) 

